Improved Algorithms for Computing the Cycle of Minimum Cost-to-Time Ratio in Directed Graphs

We study the problem of finding the cycle of minimum cost-to-time ratio in a directed graph with $ n $ nodes and $ m $ edges. This problem has a long history in combinatorial optimization and has recently seen interesting applications in the context of quantitative verification. We focus on strongly polynomial algorithms to cover the use-case where the weights are relatively large compared to the size of the graph. Our main result is an algorithm with running time $ \tilde O (m^{3/4} n^{3/2}) $, which gives the first improvement over Megiddo's $ \tilde O (n^3) $ algorithm [JACM'83] for sparse graphs. We further demonstrate how to obtain both an algorithm with running time $ n^3 / 2^{\Omega{(\sqrt{\log n})}} $ on general graphs and an algorithm with running time $ \tilde O (n) $ on constant treewidth graphs. To obtain our main result, we develop a parallel algorithm for negative cycle detection and single-source shortest paths that might be of independent interest.

==> prelim__copy_.tex <==
\section{Preliminaries}

In the following, we review some of the tools that we use in designing our algorithm.

\subsection{Parametric Search}

In the following we review the parametric search technique as outlined in~\cite{AgarwalST94}.
Assume we are given a property $ \mathcal{P} $ of real numbers that is \emph{monotone} in the following way: if $ \mathcal{P} (\lambda) $ holds, then also $ \mathcal{P} (\lambda') $ holds for all $ \lambda' < \lambda $.
Our goal is to find $ \lambda^* $, the \emph{maximum} $ \lambda $ such that $ \mathcal{P} (\lambda) $ holds.
In this paper for example, we will associate with each $ \lambda $ a weighted graph $ G_\lambda $ and $ \mathcal{P} $ is the property that $ G_\lambda $ has no negative cycle. 
Assume further that we are given an algorithm $ A $ for deciding, for a given $ \lambda $, whether $ \mathcal{P} (\lambda) $ holds.
If $ \lambda $ were known to only assume integer or rational values, we could solve this problem by performing binary search with $ O (\log{W}) $ calls to the decision algorithm, where $ W $ is the number of possible values for $ \lambda $.
However, this solution has the drawback of not yielding a strongly polynomial algorithm.

In parametric search we run the decision algorithm `generically' at the maximum $ \lambda^{*} $.
As the algorithm does not know $ \lambda^{*} $, we need to take care of its control flow ourselves and any time the algorithm performs a comparison we have to `manually' evaluate the comparison on behalf of the algorithm.
If each comparison takes the form of testing the sign of an associated low-degree polynomial $ p (\lambda) $, this can be done as follows.
We first determine all roots of $ p (\lambda) $ and check if $ \mathcal{P} (\lambda') $ holds for each such root $ \lambda' $ using another instance of the decision algorithm $ A $.
This gives us an interval between successive roots containing $ \lambda^* $ and we can thus resolve the comparison.
With every comparison we make, the interval containing $ \lambda^* $ shrinks and at the end of this process we can output a single candidate.
If the decision algorithm $ A $ has a running time of $ T $, then the overall algorithm for computing $ \lambda^* $ has a running time of $ O (T^2) $.

A more sophisticated use of the technique is possible, if in addition to a sequential decision algorithm $ A_\text{s} $ we have an efficient parallel decision algorithm $ A_\text{p} $.
The parallel algorithm performs its computations simultaneously on $ P_\text{p} $ processors.
The number of parallel computation steps until the last processor is finished is called the \emph{depth} $ D_\text{p} $ of the algorithm, and the number of operations performed by all processors in total is called the \emph{work} $ W_\text{p} $ of the algorithm.\footnote{To be precise, we use an abstract model of parallel computation as formalized in~\cite{FriedrichsL16} to avoid distraction by details such as read or write collisions typical to PRAM models.}
For parametric search, we actually only need parallelism w.r.t.\ comparisons involving the input values. %, similar to Valiant's comparison model~\cite{Valiant75}.
We denote by the \emph{comparison depth} of $ A_\text{p} $ the number of parallel comparisons (involving input values) until the last processor is finished.

We proceed similar to before:
We run $ A_\text{p} $ `generically' at the maximum $ \lambda^{*} $ and (conceptually) distribute the work among $ P_\text{p} $ processors.
Now in each parallel step, we might have to resolve up to $ P_\text{p} $ comparisons.
We first determine all roots of the polynomials associated to these comparisons.
We then perform a binary search among these roots to determine the interval of successive roots containing $ \lambda^* $ and repeat this process of resolving comparisons at every parallel step to eventually find out the value of $ \lambda^{*} $.
If the sequential decision algorithm $ A_\text{s} $ has a running time of $ T_\text{s} $ and the parallel decision algorithm runs on $ P_\text{p} $ processors in $ D_\text{p} $ parallel steps, then the overall algorithm for computing $ \lambda^* $ has a running time of $ O (P_\text{p} D_\text{p} + D_\text{p} T_\text{s} \log{P_\text{p}}) $.
Formally, the guarantees of the technique we just described can be summarized as follows.

\begin{theorem}[\cite{AgarwalST94,Megiddo83}]\label{thm:parametric search}
Let $ \mathcal{P} $ be a property of real numbers such that if $ \mathcal{P} (\lambda) $ holds, then also $ \mathcal{P} (\lambda') $ holds for all $ \lambda' < \lambda $ and let $ A_\text{p} $ and $ A_\text{s} $ be algorithms deciding for a given $ \lambda $ whether $ \mathcal{P} (\lambda) $ holds such that
\begin{itemize}
\item the control flow of $ A_\text{p} $ is only governed by comparisons that test the sign of an associated polynomial in $ \lambda $ of constant degree,
\item $ A_\text{p} $ is a parallel algorithm with work $ W_\text{p} $ and comparison depth $ D_\text{p} $, and
\item $ A_\text{s} $ is a sequential algorithm with running time $ T_\text{s} $.
\end{itemize}
Then there is a (sequential) algorithm for finding the maximum value $ \lambda $ such that $ \mathcal{P} (\lambda) $ holds with running time $ O (W_\text{p} + D_\text{p} T_\text{s} \log{W_\text{p}}) $.
\end{theorem}

Note that $ A_\text{p} $ and $ A_\text{s} $ need not necessarily be different algorithms.
In most cases however, the fastest sequential algorithm might be the better choice for minimizing running time.
%In most cases however, the running time of the best sequential algorithm is asymptotically smaller than the work of a suitable parallel algorithm.


\subsection{Characterization of Minimum Ratio Cycle}

We consider a directed graph $ G = (V, E, c, t) $, in which every edge $ e = (u, v) $ has a cost $ c (e) $ and a transit time $ t (e) $.
We want to find the cycle $ C $ that minimizes the cost-to-time ratio $ \sum_{e \in C} c (e) / \sum_{e \in C} t (e) $.

For any real $ \lambda $ define the graph $ G_\lambda = (V, E, w_\lambda) $ as the modification of $ G $ with weight $ w_\lambda (e) = c (e) - \lambda t (e) $ for every edge $ e \in E $.
The following structural lemma is the foundation of many algorithmic approaches towards the problem.

\begin{lemma}[\cite{DantzigBR67,Lawler76}]\label{lem:characterization of minimum ratio cycle}
Let $ \lambda^* $ be the value of the minimum ratio cycle of $ G $.
\begin{itemize}
\item For $ \lambda > \lambda^* $, the value of the minimum weight cycle in $ G_\lambda $ is $ < 0 $.
\item The value of the the minimum weight cycle in $ G_{\lambda^*} $ is $ 0 $. Each minimum weight cycle in $ G_{\lambda^*} $ is a minimum ratio cycle in $ G $ and vice versa.
\item For $ \lambda < \lambda^* $, the value of the minimum weight cycle in $ G_\lambda $ is $ > 0 $.
\end{itemize}
\end{lemma}

The obvious algorithmic idea now is to find the right value of $ \lambda $ with a suitable search strategy and reduce the problem to a series of negative cycle detection instances.


\subsection{Characterization of Negative Cycle}

\begin{definition}
A \emph{potential function} $ p\colon V \to \mathbb{R} $ assigns a value to each vertex of a weighted directed graph $ G = (V, E, w) $.
We call a potential function $ p $ \emph{valid} if for every edge $ e = (u, v) \in E $, the condition $ p(u) + w (e) \geq p (v) $ holds.
\end{definition}

The following two lemmas outline an approach for negative cycle detection.

\begin{lemma}[\cite{EdmondsK72}]\label{lem:negative cycle characterization}
A weighted directed graph contains a negative cycle if and only if it has no valid potential function.
\end{lemma}

\begin{lemma}[\cite{Johnson77}]\label{lem:distances give valid potential}
Let $ G = (V, E, w) $ be a weighted directed graph and let $ G' = (V', E', w') $ be the supergraph of $ G $ consisting of the vertices $ V' = V \cup \{ s' \} $ (i.e.\ with an additional super-source~$s'$), the edges $ E' = E \cup \{ s' \} \times V $ and the weight function $ w' $ given by $ w' (s', v) = 0 $ for every vertex $ v \in V $ and $ w' (u, v) = w (u, v) $ for all pairs of vertices $ u, v \in V $.
If $ G $ does not contain a negative cycle, then the potential function $ p $ defined by $ p (v) = \dist_{G'} (s', v) $ for every vertex $ v \in V $ is valid for $G$.
\end{lemma}


Thus, an obvious strategy for negative cycle detection is to design a single-source shortest paths algorithm that is correct whenever the graph contains no negative cycle.
If the graph contains no negative cycle, then the distances computed by the algorithm can be verified to be a valid potential.
If the graph does contain a negative cycle, then the distances computed by the algorithm will not be a valid potential (because a valid potential does not exist) and we can verify that the potential is not valid.


\subsection{Computing Shortest Paths in Parallel}

In our algorithm we use two building blocks for computing shortest paths in presence of negative edge weights in parallel.
The first such building block was also used by Megiddo~\cite{Megiddo83}.

\begin{observation}\label{lem:min plus}
By repeated squaring of the min-plus matrix product, all-pairs shortest paths in a directed graph with real edge weights can be computed using work $ O (n^3 \log{n}) $ and depth $ O (\log{n}) $.
\end{observation}

The second building block is a subroutine for computing the following restricted version of shortest paths.

\begin{definition}
The \emph{shortest $h$-hop path} from a vertex $ s $ to a vertex $ t $ is the path of minimum weight among all paths from $ s $ to $ t $ with at most $ h $ edges.
\end{definition}

Note that a shortest $h$-hop path from $ s $ to $ t $ does not exist, if all paths from $ s $ to $ t $ use more than $ h $ edges. 
Furthermore, if there is a shortest path from $ s $ to $ t $ with at most $ h $ edges, then the $ h $-hop shortest path from $ s $ to $ t $ is a shortest path as well.
Shortest $h$-hop paths can be computed by running $ h $ iterations of the Bellman-Ford algorithm~\cite{Ford56,Bellman58,Moore59}.\footnote{The first explicit use of the Bellman-Ford algorithm to compute shortest $h$-hop paths that we are aware of is in Thorup's dynamic APSP algorithm~\cite{Thorup05}. We would appreciate pointers to earlier uses of the Bellman-Ford algorithm for this purpose.}
Similar to shortest paths, shortest $h$-hop paths need not be unique.
We can enforce uniqueness by putting some arbitrary but fixed order on the vertices of the graph and sorting paths according to the induced lexicographic order on the sequence of vertices of the paths.
Note that the Bellman-Ford algorithm can easily be adapted to optimizing lexicographically as its second objective.

\begin{observation}\label{lem:Bellman-Ford}
By performing $ h $ iterations of the Bellman-Ford algorithm, the lexicographically smallest shortest $h$-hop path from a designated source vertex $ s $ to each other vertex in a directed graph with real edge weights can be computed using work $ O (m h) $ and depth $ O (h) $.
\end{observation}

We denote by $ \pi (s, t) $ the lexicographically smallest shortest path from $ s $ to $ t $ and by $ \pi^h (s, t) $ the lexicographically smallest shortest $h$-hop path from $ s $ to $ t $.
We denote by $ V (\pi^h (s, t)) $ and $ E (\pi^h (s, t)) $ the set of nodes and edges of $ \pi^h (s, t) $, respectively.
 

\subsection{Approximate Hitting Sets}

\begin{definition}
Given a collection of sets $ \mathcal{S} \subseteq 2^{U} $ over a universe $ U $, a hitting set is a set $ T \subseteq H $ that has non-empty intersection with every set of $ \mathcal{S} $ (i.e., $ S \cap T \neq \emptyset $ for every $ S \in \mathcal{S} $).
\end{definition}

Computing a hitting set of minimum size is an \textsf{NP}-hard problem.
For our purpose however, rough approximations are good enough.
The first method to get a sufficiently small hitting set uses a simple randomized sampling idea and was introduced to the design of graph algorithms by Ullman and Yannakakis~\cite{UllmanY91}.
We use the following formulation.

\begin{lemma}\label{lem:randomized hitting set}
Let $ c \geq 1 $, let $ U $ be a set of size $ s $ and let $ \mathcal{S} = \{ S_1, S_2, \ldots, S_k \} $ be a collection of sets over the universe $ U $ of size at least $ q $.
Let~$ T $ be a subset of $ U $ that was obtained by choosing each element of $ U $ independently with probability $ p = \min (x / q, 1) $ where $ x = c \ln{(k s)} + 1 $.
Then, with high probability (whp), i.e., probability at least $ 1 - 1/s^c $, the following two properties hold:
\begin{enumerate}
\item For every $ 1 \leq i \leq k $, the set $ S_i $ contains an element of $ T $, i.e., $ S_i \cap T \neq \emptyset $.
\item $ |T| \leq 3 x s / q = O (c s \log{(k s)} / q) $.
\end{enumerate}
\end{lemma}

The second method is to use a heuristic to compute an approximately minimum hitting set.
In the sequential model, a simple greedy algorithm computes an $ O(\log{n}) $-approximation~\cite{Johnson74a,AusielloDP80}. We use the following formulation.

\begin{lemma}\label{lem:greedy hitting set}
Let $ U $ be a set of size $ s $ and let $ \mathcal{S} = \{ S_1, S_2, \ldots, S_k \} $ be a collection of sets over the universe $ U $ of size at least $ q $.
Consider the simple greedy algorithm that picks an element $u$ in $U$ that is contained in the largest number of sets in $\mathcal{S}$ and then removes all sets containing $u$ from $\mathcal{S}$, repeating this step until $\mathcal{S} = \emptyset$.
Then the set $T$ of elements picked by this algorithm satisfies:
\begin{enumerate}
\item For every $ 1 \leq i \leq k $, the set $ S_i $ contains an element of $ T $, i.e., $ S_i \cap T \neq \emptyset $.
\item $ |T| \leq O (s \log{(k)} / q) $.
\end{enumerate}
\end{lemma}
\begin{proof}
  We follow the standard proof of the approximation ratio $O(\log n)$ for the greedy set cover heuristic. 
  The first statement is immediate, since we only remove sets when they are hit by the picked element.
  Since each of the $k$ sets contains at least $q$ elements, on average each element in $U$ is contained in at least $k q / s$ sets. Thus, the element $u$ picked by the greedy algorithm is contained in at least $k q / s$ sets. The remaining number of sets is thus at most $k - k q / s = k(1-q/s)$. Note that the remaining sets still have size at least $q$, since they do not contain the picked element $u$. Inductively, we thus obtain that after $i$ iterations the number of remaining sets is at most $k(1-q/s)^i$, so after $O(\log(k) \cdot s/q)$ iterations the number of remaining sets is less than 1 and the process stops.
\end{proof}

The above greedy algorithm is however inherently sequential and thus researchers have studied more sophisticated algorithms for the parallel model.
The state of the art in terms of deterministic algorithms is an algorithm by Berger et al.~\cite{BergerRS94}\footnote{Berger et al.\ actually give an approximation algorithm for the following slightly more general problem: Given a hypergraph $ H = (V, E) $ and a cost function $ c\colon V \to \mathbb{R} $ on the vertices, find a minimum cost subset $ R \subseteq V $ that covers $ H $, i.e., an $ R $ that minimizes $ c (R) = \sum_{v \in R} c (v) $ subject to the constraint $ e \cap R \neq \emptyset $ for all $ e \in E $.}.

\begin{theorem}[\cite{BergerRS94}]\label{thm:deterministic hitting set algorithm}
Let $ \mathcal{S} = \{ S_1, S_2, \ldots, S_k \} $ be a collection sets over the universe $ U $, let $ n = |U| $ and $ m = \sum_{1 \leq i \leq k} |S_i| $.
For $ 0 < \epsilon < 1 $, there is an algorithm with work $ O ((m + n) \epsilon^{-6} \log^4{n} \log{m} \log^6{(nm)}) $ and depth $ O (\epsilon^{-6} \log^4{n} \log{m} \log^6{(nm)}) $ that produces a hitting set of $ \mathcal{S} $ of size at most $ (1 + \epsilon) (1 + \ln{\Delta}) \cdot \mathit{OPT} $, where $ \Delta $ is the maximum number of occurrences of any element of $ U $ in $ \mathcal{S} $.
\end{theorem}

